Decoupling Training-Free Guided Diffusion by ADMM

In this paper, we consider the conditional generation problem by guiding off-the-shelf unconditional diffusion models with differentiable loss functions in a plug-and-play fashion. While previous research has primarily focused on balancing the unconditional diffusion model and the guided loss through a tuned weight hyperparameter, we propose a novel framework that distinctly decouples these two components. Specifically, we introduce two variables ${x}$ and ${z}$, to represent the generated samples governed by the unconditional generation model and the guidance function, respectively. This decoupling reformulates conditional generation into two manageable subproblems, unified by the constraint ${x} = {z}$. Leveraging this setup, we develop a new algorithm based on the Alternating Direction Method of Multipliers (ADMM) to adaptively balance these components. Additionally, we establish the equivalence between the diffusion reverse step and the proximal operator of ADMM and provide a detailed convergence analysis of our algorithm under certain mild assumptions. Our experiments demonstrate that our proposed method ADMMDiff consistently generates high-quality samples while ensuring strong adherence to the conditioning criteria. It outperforms existing methods across a range of conditional generation tasks, including image generation with various guidance and controllable motion synthesis.

==> tables/22_nip_imagenet_fid_lpips.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{lllllllllll}
\toprule
{} & \multicolumn{2}{c}{\textbf{SR ($\times 4$)}} & \multicolumn{2}{c}{\textbf{Inpaint (box)}} & \multicolumn{2}{c}{\textbf{Inpaint (random)}} &
\multicolumn{2}{c}{\textbf{Deblur (gauss)}} & \multicolumn{2}{c}{\textbf{Deblur (motion)}}\\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
{\textbf{Method}} & {FID $\downarrow$} & {LPIPS $\downarrow$} & {FID $\downarrow$} & {LPIPS $\downarrow$} & {FID $\downarrow$} & {LPIPS $\downarrow$} & {FID $\downarrow$} & {LPIPS $\downarrow$} & {FID $\downarrow$} & {LPIPS $\downarrow$}\\
\midrule


ADMM-TV & 130.9 & 0.523 & 87.69 & 0.319 & 189.3 & 0.510 & 155.7 & 0.588 & 138.8 & 0.525 \\
Score-SDE~\citep{song_2020_score} & 170.7 & 0.701 & 54.07 & 0.354 & 127.1 & 0.659 & 120.3 & 0.667 & 98.25 & 0.591 \\
PnP-ADMM~\citep{chan2016plug} & 97.27 & 0.433 & 78.24 & 0.367 & 114.7 & 0.677 & 100.6 & 0.519 & 89.76 & 0.483 \\
MCG~\citep{chung2022improving} & 144.5 & 0.637 & 39.74 & 0.330 & 39.19 & 0.414 & 95.04 & 0.550 & 186.9 & 0.758 \\
DDRM~\citep{kawar2022denoising} & 59.57 & 0.339 & 45.95 & \textbf{0.245} & 114.9 & 0.665 & 63.02 & \underline{0.427} & - & -\\
DPS~\citep{chung2022diffusion} & \underline{50.66} & \underline{0.337} & \underline{38.82} & \underline{0.262} & \underline{35.87} & \underline{0.303} & \underline{62.72} & 0.444 & \underline{56.08} & \underline{0.389} \\
\textbf{ADMMDiff} & \textbf{49.97} & \textbf{0.331} & \textbf{37.47} & \underline{0.262} & \textbf{34.80} & \textbf{0.207} & \textbf{51.3} & \textbf{0.414} &\textbf{55.99} & \textbf{0.364}\\


\bottomrule
\end{tabular}
}
\caption{
Quantitative evaluation (FID, LPIPS) of solving linear inverse problems on ImageNet 256$\times$256-1k validation dataset. \textbf{Bold} indicates the best. \underline{Underline} indicates the second best.
}
\vspace{-1.5em}
\label{tab:nip_imagenet_fid_lpips}
\end{table*}

